Super-Resolution Estimation of UWB Channels including the Diffuse Component -- An SBL-Inspired Approach

In this paper, we present an iterative algorithm that detects and estimates the specular components and estimates the diffuse component of single-input-multiple-output (SIMO) ultra-wide-band (UWB) multipath channels. Specifically, the algorithm super-resolves the specular components in the delay-angle-of-arrival domain and estimates the parameters of a parametric model of the delay-angle power spectrum characterizing the diffuse component. Channel noise is also estimated. In essence, the algorithm solves the problem of estimating spectral lines (the specular components) in colored noise (generated by the diffuse component and channel noise). Its design is inspired by the sparse Bayesian learning (SBL) framework. As a result the iteration process contains a threshold condition that determines whether a candidate specular component shall be retained or pruned. By relying to results from extreme-value analysis the threshold of this condition is suitably adapted to ensure a prescribed probability of detecting spurious specular components. Studies using synthetic and real channel measurement data demonstrate the virtues of the algorithm: it is able to still detect and accurately estimate specular components, even when their separation in delay and angle is down to half the Rayleigh resolution limit (RRL) of the equipment; it is robust in the sense that it tends to return no more specular components than the actual ones. Finally, the algorithm is shown to outperform a state-of-the-art super-resolution channel estimator.

==> definitions.tex <==
% Extend acronym package with first letter caps
\makeatletter
\newif\ifAC@uppercase@first%
\def\Aclp#1{\AC@uppercase@firsttrue\aclp{#1}\AC@uppercase@firstfalse}%
\def\AC@aclp#1{%
	\ifcsname fn@#1@PL\endcsname%
	\ifAC@uppercase@first%
	\expandafter\expandafter\expandafter\MakeUppercase\csname fn@#1@PL\endcsname%
	\else%
	\csname fn@#1@PL\endcsname%
	\fi%
	\else%
	\AC@acl{#1}s%
	\fi%
}%
\def\Acp#1{\AC@uppercase@firsttrue\acp{#1}\AC@uppercase@firstfalse}%
\def\AC@acp#1{%
	\ifcsname fn@#1@PL\endcsname%
	\ifAC@uppercase@first%
	\expandafter\expandafter\expandafter\MakeUppercase\csname fn@#1@PL\endcsname%
	\else%
	\csname fn@#1@PL\endcsname%
	\fi%
	\else%
	\AC@ac{#1}s%
	\fi%
}%
\def\Acfp#1{\AC@uppercase@firsttrue\acfp{#1}\AC@uppercase@firstfalse}%
\def\AC@acfp#1{%
	\ifcsname fn@#1@PL\endcsname%
	\ifAC@uppercase@first%
	\expandafter\expandafter\expandafter\MakeUppercase\csname fn@#1@PL\endcsname%
	\else%
	\csname fn@#1@PL\endcsname%
	\fi%
	\else%
	\AC@acf{#1}s%
	\fi%
}%
\def\Acsp#1{\AC@uppercase@firsttrue\acsp{#1}\AC@uppercase@firstfalse}%
\def\AC@acsp#1{%
	\ifcsname fn@#1@PL\endcsname%
	\ifAC@uppercase@first%
	\expandafter\expandafter\expandafter\MakeUppercase\csname fn@#1@PL\endcsname%
	\else%
	\csname fn@#1@PL\endcsname%
	\fi%
	\else%
	\AC@acs{#1}s%
	\fi%
}%
\edef\AC@uppercase@write{\string\ifAC@uppercase@first\string\expandafter\string\MakeUppercase\string\fi\space}%
\def\AC@acrodef#1[#2]#3{%
	\@bsphack%
	\protected@write\@auxout{}{%
		\string\newacro{#1}[#2]{\AC@uppercase@write #3}%
	}\@esphack%
}%
\def\Acl#1{\AC@uppercase@firsttrue\acl{#1}\AC@uppercase@firstfalse}
\def\Acf#1{\AC@uppercase@firsttrue\acf{#1}\AC@uppercase@firstfalse}
\def\Ac#1{\AC@uppercase@firsttrue\ac{#1}\AC@uppercase@firstfalse}
\def\Acs#1{\AC@uppercase@firsttrue\acs{#1}\AC@uppercase@firstfalse}
\robustify\Aclp
\robustify\Acfp
\robustify\Acp
\robustify\Acsp
\robustify\Acl
\robustify\Acf
\robustify\Ac
\robustify\Acs
\makeatother 

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Math

\newtheorem{prop}{Proposition}
\newtheorem{remark}{Remark}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}
\newtheorem{assumption}{Assumption}
\newtheorem{conjecture}{Conjecture}

\newcommand{\vu}[2]{\mbox{$#1\,\text{#2}$}} % "value~unit" ... prevents e.g. 456 \linebreak mV
\newcommand{\diag}[1]{\text{diag}}   %identity matrix
\newcommand{\argmin}[1]{\underset{#1}{\text{arg\,min}}}
\newcommand{\argmax}[1]{\underset{#1}{\text{arg\,max}}}
\newcommand{\trans}{^{\text{T}}}
\newcommand{\herm}{^{\text{H}}}
\newcommand{\inprod}[2]{\ensuremath{\bigl\langle #1 \bigr\rangle_{#2}}}%inner product

\newcommand{\mtx}[2]{\left[\ensuremath{\begin{array}{#1}#2\end{array}}\right]}%vector/matrix
\newcommand{\mtxt}[1]{\ensuremath{\bigl[\,#1\,\bigr]}}%vector/matrix for inline definition

\DeclareRobustCommand{\BM}[1]{%
  \ifcat\noexpand#1\relax\bm{\boldUppercaseItalicGreek{#1}}\else\bm{#1}\fi
}
\newcommand{\V}[1]{\bm{#1}}
\newcommand{\M}[1]{\BM{#1}}
\DeclareRobustCommand{\mcal}[1]{%
  \ifcat\noexpand#1\relax\mathnormal{#1}\else\cal{#1}\fi
}
\newcommand{\Set}[1]{{\mcal{#1}}}
\makeatletter
\newcommand{\boldUppercaseItalicGreek}[1]{\csname var\expandafter\@gobble\string#1\endcsname}
\makeatother


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Special Symbols
\newcommand{\SNR}{\mathrm{SNR}}
\newcommand{\SIR}{\mathrm{SIR}}
\newcommand{\SINR}{\mathrm{SINR}}
\newcommand{\SDR}{\mathrm{SDR}}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% table
\newcommand{\thead}[1]{\multicolumn{1}{c|}{#1}}
\renewcommand{\arraystretch}{1.1}
\newcolumntype{R}{>{\raggedleft\arraybackslash}X}%
%\newcolumntype{L}{>{\raggedright\arraybackslash}X}%
%\newcolumntype{C}{>{\centering\arraybackslash}X}%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Algorithm new Counter
\makeatletter
\newcounter{myproc}
\newenvironment{myproc}[1][htb]
  {\renewcommand{\algorithmcfname}{Procedure}% Update algorithm name
   \let\c@algocf\c@myproc% Update algorithm counter
   \begin{algorithm}[#1]%
  }{\end{algorithm}}
\makeatother
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% PGF Stuff
\usetikzlibrary{calc,arrows.meta}
\ifthenelse{\equal{\exportFigures}{true}}
{
  \usepgfplotslibrary{external}\tikzexternalize[prefix=\tikzfolder]
%   \tikzset{
%     png export/.style={
%       external/system call={
%         pdflatex \tikzexternalcheckshellescape -halt-on-error -interaction=batchmode -jobname "\image" "\texsource";
%         convert -density 300 -transparent white "\image.pdf" "\image.png";
% %         dvips -o "\image".ps "\image".dvi;
% %         ps2eps "\image.ps"
%       }
%     }
%   }
%   \tikzset{png export}
}
{}

% argument #1: any options
\newenvironment{customlegend}[1][]{%
    \begingroup
    % inits/clears the lists (which might be populated from previous
    % axes):
    \csname pgfplots@init@cleared@structures\endcsname
    \pgfplotsset{#1}%
}{%
    % draws the legend:
    \csname pgfplots@createlegend\endcsname
    \endgroup
}%

% makes \addlegendimage available (typically only available within an
% axis environment):
\def\addlegendimage{\csname pgfplots@addlegendimage\endcsname}
\def\addlegendentry{\csname pgfplots@addlegendentry\endcsname}


\newcommand{\pgfref}[1]
{\ifthenelse{\equal{\exportFigures}{true}}
{\tikzexternaldisable\ref{#1}\tikzexternalenable}
{\ref{#1}}}
% \newcommand{\pgfref}[1]
% {\ifthenelse{\equal{\exportFigures}{true}}
% {\tikzset{external/export=false}\protect\ref{#1}\tikzset{external/export=true}}
% {\protect\ref{#1}}}

\pgfplotsset{compat=newest} 

\newlength\figureheight 
\newlength\figurewidth 
\usetikzlibrary{patterns,arrows}
\usepgfplotslibrary{colormaps}
\usetikzlibrary{plotmarks}
\pgfplotsset{every axis/.append style={
  label style={font=\footnotesize},
  tick label style={font=\tiny},
  xticklabel={
   % test if the x value is below zero
   \ifdim \tick pt < 0pt
    % if yes, calculate the absolute value
    \pgfmathparse{abs(\tick)}%
    % and print first a minus sign in a zero-width box, followed by the absolute value
    \llap{$-{}$}\pgfmathprintnumber{\pgfmathresult}
   \else
    % if no, print as usual
    \pgfmathprintnumber{\tick}
   \fi}
   }}
\usetikzlibrary{decorations.markings}
\makeatletter
\tikzset{
  nomorepostactions/.code={\let\tikz@postactions=\pgfutil@empty},
  mymarkfixednumber/.style n args={3}{decoration={markings,
    mark= between positions 0 and 1 step (1/#3)*\pgfdecoratedpathlength with{%
        \tikzset{#2,every mark}\tikz@options
        \pgftransformresetnontranslations%
        \pgfuseplotmark{#1}%
      },  
    },
    postaction={decorate},
    /pgfplots/legend image post style={
        mark=#1,mark options={#2},every path/.append style={nomorepostactions}
    },
  },
}
\tikzset{
  nomorepostactions/.code={\let\tikz@postactions=\pgfutil@empty},
  mymarkfixeddistance/.style n args={3}{decoration={markings,
    mark= between positions 0 and 1 step #3cm with{%
        \tikzset{#2,every mark}\tikz@options
        \pgftransformresetnontranslations%
        \pgfuseplotmark{#1}%
      },  
    },
    postaction={decorate},
    /pgfplots/legend image post style={
        mark=#1,mark options={#2},every path/.append style={nomorepostactions}
    },
  },
}
\tikzset{
  nomorepostactions/.code={\let\tikz@postactions=\pgfutil@empty},
  mymark/.style n args={3}{decoration={markings,
    mark= between positions 0 and 1 step 0.75cm with{%
        \tikzset{#2,every mark}\tikz@options
        \pgftransformresetnontranslations%
        \pgfuseplotmark{#1}%
      },  
    },
    postaction={decorate},
    /pgfplots/legend image post style={
        mark=#1,mark options={#2},every path/.append style={nomorepostactions}
    },
  },
}
% \tikzset{
%   nomorepostactions/.code={\let\tikz@postactions=\pgfutil@empty},
%   mymark/.style 2 args={decoration={markings,
%     mark= between positions 0 and 1 step (1/20)*\pgfdecoratedpathlength with{%
%         \tikzset{#2,every mark}\tikz@options
%         \pgfuseplotmark{#1}%
%       },  
%     },
%     postaction={decorate},
%     /pgfplots/legend image post style={
%         mark=#1,mark options={solid},every path/.append style={nomorepostactions}
%     },
%   },
% }
\makeatother

% Plot Pa Pm
\definecolor{colA}{rgb}{0,0,1}% blue 
\definecolor{colB}{rgb}{1.00000,0.0,0.00000}% red
\definecolor{colC}{rgb}{0,0.7,0}% green
\definecolor{colD}{rgb}{0.9,0.0,0.9}% magenta
\definecolor{colE}{rgb}{0,1,1}% cyan
\definecolor{colF}{rgb}{1.00000,0.55,0.00000}% dark-orange

\def\mylinewidth{0.4}

\def\mymarksize{1.5}
\def\markA{o}
\def\markB{square}
\def\markC{triangle}
\def\markD{diamond}
\def\markE{pentagon}
\def\markF{+}

\pgfplotsset{Pa/.style={solid, line width=\mylinewidth}}
\pgfplotsset{Pa_theory/.style={dashed, line width=\mylinewidth}}
\pgfplotsset{Pm/.style={densely dotted, line width=\mylinewidth}}
\pgfplotsset{Pm_theory/.style={dash dot, line width=\mylinewidth}}

\pgfplotsset{snr1/.style={color=colA, mymarkfixeddistance={\markA}{mark size=\mymarksize,solid}{1}}}
\pgfplotsset{snr2/.style={color=colB, mymarkfixeddistance={\markB}{mark size=\mymarksize,solid}{1}}}
\pgfplotsset{snr3/.style={color=colC, mymarkfixeddistance={\markC}{mark size=\mymarksize,solid}{1}}}

% \pgfplotsset{snr1_Pa/.style={color=colA, solid, line width=\mylinewidth, mark size=\mymarksize, mark=\markA, mark repeat=1, mark phase = 0, mark options={solid}}}
\pgfplotsset{snr1_Pa/.style={color=colA, solid, line width=\mylinewidth, mymarkfixeddistance={\markA}{mark size=\mymarksize,solid}{1}}}
\pgfplotsset{snr1_Pa_theory/.style={color=colA, dashed, line width=\mylinewidth, mymarkfixeddistance={\markA}{mark size=\mymarksize,solid}{1}}}
\pgfplotsset{snr1_Pm/.style={color=colA, densely dotted, line width=\mylinewidth, mymarkfixeddistance={\markA}{mark size=\mymarksize,solid}{1}}}
\pgfplotsset{snr1_Pm_theory/.style={color=colA, dash dot, line width=\mylinewidth, mymarkfixeddistance={\markA}{mark size=\mymarksize,solid}{1}}}

% \pgfplotsset{snr2_Pa/.style={color=colB, solid, line width=\mylinewidth, mark size=\mymarksize, mark=\markB, mark repeat=1, mark phase = 0, mark options={solid}}}
\pgfplotsset{snr2_Pa/.style={color=colB, solid, line width=\mylinewidth, mymarkfixeddistance={\markB}{mark size=\mymarksize,solid}{1}}}
\pgfplotsset{snr2_Pa_theory/.style={color=colB, dashed, line width=\mylinewidth, mymarkfixeddistance={\markB}{mark size=\mymarksize,solid}{1}}}
\pgfplotsset{snr2_Pm/.style={color=colB, densely dotted, line width=\mylinewidth, mymarkfixeddistance={\markB}{mark size=\mymarksize,solid}{1}}}
\pgfplotsset{snr2_Pm_theory/.style={color=colB, dash dot, line width=\mylinewidth, mymarkfixeddistance={\markB}{mark size=\mymarksize,solid}{1}}}

% \pgfplotsset{snr3_Pa/.style={color=colC, solid, line width=\mylinewidth, mark size=\mymarksize, mark=\markC, mark repeat=1, mark phase = 0, mark options={solid}}}
\pgfplotsset{snr3_Pa/.style={color=colC, solid, line width=\mylinewidth, mymarkfixeddistance={\markC}{mark size=\mymarksize,solid}{1}}}
\pgfplotsset{snr3_Pa_theory/.style={color=colC, dashed, line width=\mylinewidth, mymarkfixeddistance={\markC}{mark size=\mymarksize,solid}{1}}}
\pgfplotsset{snr3_Pm/.style={color=colC, densely dotted, line width=\mylinewidth, mymarkfixeddistance={\markC}{mark size=\mymarksize,solid}{1}}}
\pgfplotsset{snr3_Pm_theory/.style={color=colC, dash dot, line width=\mylinewidth, mymarkfixeddistance={\markC}{mark size=\mymarksize,solid}{1}}}

% \pgfplotsset{snr4_Pa_unknown/.style={color=colD, solid, line width=\mylinewidth, mark size=\mymarksize, mark=\markD, mark repeat=1, mark phase = 0, mark options={solid}}}
% \pgfplotsset{snr4_Pa_theory/.style={color=colD, dashed, line width=\mylinewidth, mark size=\mymarksize, mark=\markD, mark repeat=1, mark phase = 0, mark options={solid}}}
% \pgfplotsset{snr4_Pm_unknown/.style={color=colD, dashed, line width=\mylinewidth, mark size=\mymarksize, mark=\markD, mark repeat=1, mark phase = 0, mark options={solid}}}
% \pgfplotsset{snr4_Pm_known/.style={color=colD, dash dot, line width=\mylinewidth, mark size=\mymarksize, mark=\markD, mark repeat=1, mark phase = 0, mark options={solid}}}
% \pgfplotsset{snr4_Pm_theory/.style={color=colD, solid, line width=\mylinewidth, mark size=\mymarksize, mark=none, mark repeat=1, mark phase = 0, mark options={solid}}}
% 
% \pgfplotsset{snr5_Pa_unknown/.style={color=colE, solid, line width=\mylinewidth, mark size=\mymarksize, mark=\markE, mark repeat=1, mark phase = 0, mark options={solid}}}
% \pgfplotsset{snr5_Pa_theory/.style={color=colE, dashed, line width=\mylinewidth, mark size=\mymarksize, mark=\markE, mark repeat=1, mark phase = 0, mark options={solid}}}
% \pgfplotsset{snr5_Pm_unknown/.style={color=colE, dashed, line width=\mylinewidth, mark size=\mymarksize, mark=\markE, mark repeat=1, mark phase = 0, mark options={solid}}}
% \pgfplotsset{snr5_Pm_known/.style={color=colE, dash dot, line width=\mylinewidth, mark size=\mymarksize, mark=\markE, mark repeat=1, mark phase = 0, mark options={solid}}}
% \pgfplotsset{snr5_Pm_theory/.style={color=colE, solid, line width=\mylinewidth, mark size=\mymarksize, mark=none, mark repeat=1, mark phase = 0, mark options={solid}}}
% 
% \pgfplotsset{snr6_Pa_unknown/.style={color=colF, solid, line width=\mylinewidth, mark size=\mymarksize, mark=\markF, mark repeat=1, mark phase = 0, mark options={solid}}}
% \pgfplotsset{snr6_Pa_theory/.style={color=colF, dashed, line width=\mylinewidth, mark size=\mymarksize, mark=\markF, mark repeat=1, mark phase = 0, mark options={solid}}}
% \pgfplotsset{snr6_Pm_unknown/.style={color=colF, dashed, line width=\mylinewidth, mark size=\mymarksize, mark=\markF, mark repeat=1, mark phase = 0, mark options={solid}}}
% \pgfplotsset{snr6_Pm_known/.style={color=colF, dash dot, line width=\mylinewidth, mark size=\mymarksize, mark=\markF, mark repeat=1, mark phase = 0, mark options={solid}}}
% \pgfplotsset{snr6_Pm_theory/.style={color=colF, solid, line width=\mylinewidth, mark size=\mymarksize, mark=none, mark repeat=1, mark phase = 0, mark options={solid}}}

\pgfplotsset{snr_Pa_known/.style={color=black, solid, line width=\mylinewidth, mark size=\mymarksize, mark=heart, mark repeat=1, mark phase = 0, mark options={solid}}}
\pgfplotsset{snr_Pa_known_theory/.style={color=black, solid, line width=\mylinewidth, mark size=\mymarksize, mark=none, mark repeat=1, mark phase = 0, mark options={solid}}}

\pgfplotsset{TypeII/.append style={mymark={*}{solid,fill opacity=0.0}{}}}
\pgfplotsset{TypeI_Nadler/.append style={mymark={triangle*}{solid,fill opacity=0.0}{}}}
\pgfplotsset{knownC_TypeII/.append style={mymark={*}{solid,fill opacity=0.0}{}}}
\pgfplotsset{knownC_TypeI_Nadler/.append style={mymark={triangle*}{solid,fill opacity=0.0}{}}}
\pgfplotsset{AtomicNormSoftThresholdMEMP/.append style={mymark={triangle*}{solid,fill opacity=0.0}{}}}
\pgfplotsset{AtomicNormSoftThresholdMEMP_Imax10/.append style={mymark={triangle*}{solid,fill opacity=0.0}{}}}
\pgfplotsset{MEMP/.append style={mymark={diamond*}{solid,fill opacity=0.0}{}}}

\pgfplotsset{dist/.style={colA, solid, line width=\mylinewidth,mark size=\mymarksize}}
\pgfplotsset{dist_crlb/.style={colA, solid, line width=0.2,mark size=\mymarksize,mymark={asterisk}{solid}{}}}
\pgfplotsset{axis_dist/.style={color=colA}}

\pgfplotsset{aoa/.style={colB, dashed, line width=\mylinewidth,mark size=\mymarksize, mark repeat=1, mark phase = 0, mark options={solid}}}
\pgfplotsset{aoa_crlb/.style={colB, dashed, line width=0.2,mark size=\mymarksize,mymark={asterisk}{solid}{}}}
\pgfplotsset{axis_aoa/.style={color=colB, /pgf/number format/.cd,precision=0,fixed,/tikz/.cd}}

% \pgfplotsset{K_d/.style={color=colC, line width=\mylinewidth, mark=\markC, mark size=\mymarksize, mark repeat=1, mark phase = 0, mark options={solid}}}
% \pgfplotsset{axis_K_d/.style={color=colC}}
% 
% \pgfplotsset{P_d/.style={color=colD, solid, line width=\mylinewidth, mark=\markD, mark size=\mymarksize, mark repeat=1, mark phase = 0, mark options={solid}}}
% \pgfplotsset{axis_P_d/.style={color=colD}}
% 
% \pgfplotsset{rmse_d/.style={color=colB, line width=\mylinewidth, mark size=\mymarksize, mark=\markA, mark repeat=1, mark phase = 0, mark options={solid, colB}}}
% \pgfplotsset{crlb_d/.style={color=colB, dotted, line width=\mylinewidth, mark size=\mymarksize, mark=\markA, mark repeat=1, mark phase = 0, mark options={solid, colB}}}
% \pgfplotsset{axis_d/.style={color=colB}}
% 
% \pgfplotsset{rmse_aoa/.style={color=colA, line width=\mylinewidth, mark size=\mymarksize, mark=\markB, mark repeat=1, mark phase = 0, mark options={solid, colA}}}
% \pgfplotsset{crlb_aoa/.style={color=colA, dotted, line width=\mylinewidth, mark size=\mymarksize, mark=\markB, mark repeat=1, mark phase = 0, mark options={solid, colA}}}
% \pgfplotsset{axis_aoa/.style={color=colA}}



% \pgfplotsset{TypeII/.append style={solid}}
% \pgfplotsset{TypeI/.append style={dashed}}
% \pgfplotsset{TypeI_Nadler/.append style={dashed}}
% \pgfplotsset{TypeI_Nadler_old/.append style={dash pattern={on 3pt off 1pt on 0.5pt off 1pt}}}
% \pgfplotsset{TypeI_Wald/.append style={dash pattern={on 3pt off 1pt on 0.5pt off 1pt}}}
% \pgfplotsset{TypeI_Factorized/.append style={dashed}}
% 
% \pgfplotsset{K_d/.style={color=colC, line width=\mylinewidth, mark=\markC, mark size=\mymarksize, mark repeat=1, mark phase = 0, mark options={solid}}}
% \pgfplotsset{axis_K_d/.style={color=colC}}
% 
% \pgfplotsset{P_d/.style={color=colD, solid, line width=\mylinewidth, mark=\markD, mark size=\mymarksize, mark repeat=1, mark phase = 0, mark options={solid}}}
% \pgfplotsset{axis_P_d/.style={color=colD}}
% 
% \pgfplotsset{rmse_d/.style={color=colB, line width=\mylinewidth, mark size=\mymarksize, mark=\markA, mark repeat=1, mark phase = 0, mark options={solid, colB}}}
% \pgfplotsset{crlb_d/.style={color=colB, dotted, line width=\mylinewidth, mark size=\mymarksize, mark=\markA, mark repeat=1, mark phase = 0, mark options={solid, colB}}}
% \pgfplotsset{axis_d/.style={color=colB}}
% 
% \pgfplotsset{rmse_aoa/.style={color=colA, line width=\mylinewidth, mark size=\mymarksize, mark=\markB, mark repeat=1, mark phase = 0, mark options={solid, colA}}}
% \pgfplotsset{crlb_aoa/.style={color=colA, dotted, line width=\mylinewidth, mark size=\mymarksize, mark=\markB, mark repeat=1, mark phase = 0, mark options={solid, colA}}}
% \pgfplotsset{axis_aoa/.style={color=colA}}

